Correlating power consumption and network traffic for improving data centers resiliency

The deployment of business critical applications and information infrastructures are moving to the cloud. This means they are hosted in large scale data centers with other business applications and infrastructures with less (or none) mission critical constraints. This mixed and complex environment makes very challenging the process of monitoring critical applications and handling (detecting and recovering) possible failures of servers' data center that could affect responsiveness and/or reliability of mission critical applications. Monitoring mechanisms used in data center are usually intrusive in the sense that they need to install agents on each single server. This has considerable drawbacks: huge usage of human resources to install and patch the system and interference with the critical application because agents share application resources. In order to detect (and possibly predict) failures in data centers the paper does a first attempt in showing the correlation between network traffic and servers' power consumption. This is an important step in deriving non-intrusive monitoring systems, as both network traffic and power consumption can be captured without installing any software at the servers. This will improve in its turn the overall resiliency of the data center and its self-managing capacity.

==> environment.tex <==
% !TEX root = main.tex
\section{Environment}
